JI-ADF: Joint-Individual Learning with Adaptive Decision Fusion for Multimodal Skin Lesion Classification

Skin lesion classification is essential for early dermatological diagnosis, yet many existing computer-aided systems rely primarily on dermoscopic images and underutilize the multimodal evidence routinely available in clinical practice. To address this gap, we propose \textbf{JI-ADF}, a trimodal deep learning framework that integrates dermoscopic images, clinical photographs, and structured patient metadata for clinically grounded skin lesion classification. The proposed architecture combines joint multimodal representation learning with modality-specific auxiliary supervision and an adaptive decision fusion mechanism that dynamically calibrates modality contributions on a per-sample basis. To enhance cross-modal reasoning while preserving modality-specific evidence, we further introduce a multimodal fusion attention (MMFA) module. We evaluate JI-ADF on the large-scale MILK10k benchmark, which reflects real-world clinical acquisition conditions and severe class imbalance. The proposed method demonstrates strong and well-balanced performance across lesion categories, improving sensitivity and Dice score while maintaining high specificity and good calibration. Extensive analyses, including modality ablation, calibration evaluation, and Grad-CAM visualization, further confirm the robustness and clinically meaningful behavior of the model. These results indicate that JI-ADF provides a reliable and practical foundation for multimodal skin lesion classification in real-world clinical settings.

==> sec/2_related.tex <==
\section{Related Work}
\label{sec:related}

\subsection{Skin lesion classification based on images}

In recent years, deep learning has become the leading approach for skin lesion classification (SLC), particularly through convolutional neural networks that have consistently dominated ISIC challenges since 2016. A very deep residual CNN achieved the top performance in the ISIC 2016 skin lesion classification challenge among 25 teams \cite{7792699}, marking a significant milestone for automated melanoma recognition. Building on this success, a series of state-of-the-art CNN-based frameworks have been proposed for the SLC task \cite{9018274, TANG2019289, 8990108, 8578235, JIN2021106881}. Among them, \cite{9018274} introduced a GP-CNN-DTEL architecture that captures both global and local representations via data-transformed ensemble learning, achieving strong results in melanoma and nevus classification. To further enhance performance, \cite{8990108} proposed a mutual bootstrapping strategy that jointly benefits segmentation and classification, reporting a Jaccard index of 80.4\% for segmentation and an average AUC of 93.8\% for classification on the ISIC 2017 dataset. Additionally, \cite{WANG2021108075} designed a cascade knowledge diffusion network that transfers and fuses features learned from lesion segmentation models to improve SLC accuracy. Other works explored combining dermoscopic and clinical images for skin disease recognition \cite{BI2020107502, 10.1007.978-3-319-66179-7_29}, while comparative studies between CNN-based systems and medical experts showed that deep models can achieve diagnostic accuracy comparable to or exceeding that of most dermatologists \cite{Esteva2017, Haenssle2018, BRINKER201947, BARATA2021107413}.

\subsection{Skin lesion classification based on the fusion of images and metadata}

Multimodal fusion aims to integrate heterogeneous sources of information so that complementary cues can be jointly exploited for learning tasks \cite{Atrey2010}. Compared with single-modality models, such fusion strategies often provide richer representations and improved predictive performance \cite{Huang2020}. Encouraged by successes in other domains, where combining visual and textual or sensor data significantly boosts accuracy \cite{10.1117.12.2501679, 10.1115.1.4043222}, researchers have increasingly explored multimodal learning for medical image analysis, including dermatology \cite{Huang2020}.

In clinical practice, dermatologists rarely rely on images alone. Patient demographics and clinical context, such as age, sex, lesion location, and medical history, often play a decisive role when visual patterns are ambiguous. This has motivated a growing body of work that combines dermoscopic images with patient metadata for skin lesion classification \cite{Yap2018, 8333693, Liu2020, 9364366, 9098645}. Early attempts demonstrated the feasibility of deep learning models that jointly process dermatological images and tabular information \cite{Yap2018}. Subsequent studies extended this idea by designing dedicated multimodal networks for multi-label recognition \cite{8333693} and by incorporating multi-view images together with metadata to improve differential diagnosis performance \cite{Liu2020}. Notably, these systems were reported to achieve dermatologist-level accuracy in certain evaluation settings.

Despite these encouraging results, many existing approaches rely on straightforward feature concatenation to merge modalities, which may fail to capture complex cross-modal dependencies \cite{PACHECO2020103545, 9098645}. To address this limitation, later works explored attention-driven mechanisms to better exploit modality interactions. Methods such as Metablock, Metanet, and Mutual Attention attempt to highlight the most informative visual cues under the guidance of metadata and have shown improved performance over naive concatenation schemes \cite{9364366, Liu2020, Cai2023}.

However, most current designs still employ a joint fusion paradigm that compresses multimodal inputs into a single shared representation. Such strategies may overlook modality-specific characteristics that are important for dermatological analysis \cite{9363019, 8027090}. Moreover, many fusion modules primarily use metadata to refine image features, rather than modeling bidirectional interactions between modalities. These limitations suggest that more adaptive and structurally aware fusion mechanisms remain necessary for robust skin lesion classification.

==> sec/4_experiments.tex <==
\section{Experiments}
We now first describe our experimental set-up before reporting and discussing the results.

% \subsection{Dataset Description}
\subsection{Dataset Description} 
We used the MILK10k multimodal skin-lesion dataset \cite{Tschandl2025MILK10k} to train and evaluate our method. The MILK10k dataset contains 10480 images from 5240 lesions, provided as paired clinical close-up and dermoscopic images collected across five centers. For testing, we follow the official hidden test comprising 479 lesions with paired images (958 images), provided with the metadata fields as the training set. This data can be found here: \url{https://challenge.isic-archive.com/data/#milk10k}.

\begin{table}[ht]
\centering
\small
\renewcommand{\arraystretch}{1.2}
\setlength{\tabcolsep}{8pt}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcc}
\toprule
\textbf{Diagnostic Category} & \textbf{Abbreviation} & \textbf{Quantity (training set)} \\
\midrule
Actinic keratosis/intraepidermal carcinoma & AKIEC & 242 \\
Basal cell carcinoma & BCC & 2017 \\
Other benign proliferations including collisions & BEN\_OTH & 35 \\
Benign keratinocytic lesion & BKL & 435 \\
Dermatofibroma & DF & 42 \\
Inflammatory and infectious & INF & 40 \\
Other malignant proliferations including collisions & MAL\_OTH & 7 \\
Melanoma & MEL & 360 \\
Melanocytic nevus, any type & NV & 597 \\
Squamous cell carcinoma/keratoacanthoma & SCCKA & 379 \\
Vascular lesions and hemorrhage & VASC & 38 \\
\bottomrule
\end{tabular}
}
\caption{Distribution of diagnostic categories in the training set.}
\label{tab:data_distribution}
\end{table}


\subsection{Implementation}

% \cite{loshchilov2019decoupledweightdecayregularization}

Our model was trained for 50 epochs with a batch size of $16$, using AdamW optimizer \cite{loshchilov2019decoupledweightdecayregularization} with the initial learning rate value of 1e-4 and weight decay of 1e-5. The ReduceLROnPlateau scheduler is applied for the learning rate decay. We split the training set into 80\% for training and 20\% for validation. The model achieving the highest average Macro F1 Score on the validation set was saved for testing. The ImageNet-1K \cite{5206848} pretrained EfficientNetV2 is employed as the backbone. Input images are resized to $384 \times 384 \times 3$, the length of the encoded patient's metadata is $256$, and we use MMFA (Section~\ref{sec:MMFA}) to fuse images and metadata features. All the experiments were performed using Python 3.12 with PyTorch 2.8.0 and run on NVIDIA A100 GPU with 40GB VRAM.
